Efficient Large Language Models: A Survey

Large Language Models (LLMs) have demonstrated remarkable capabilities in important tasks such as natural language understanding and language generation, and thus have the potential to make a substantial impact on our society. Such capabilities, however, come with the considerable resources they demand, highlighting the strong need to develop effective techniques for addressing their efficiency challenges. In this survey, we provide a systematic and comprehensive review of efficient LLMs research. We organize the literature in a taxonomy consisting of three main categories, covering distinct yet interconnected efficient LLMs topics from model-centric, data-centric, and framework-centric perspective, respectively. We have also created a GitHub repository where we organize the papers featured in this survey at https://github.com/AIoT-MLSys-Lab/Efficient-LLMs-Survey. We will actively maintain the repository and incorporate new research as it emerges. We hope our survey can serve as a valuable resource to help researchers and practitioners gain a systematic understanding of efficient LLMs research and inspire them to contribute to this important and exciting field.

==> Section/1_Introduction_BACKUP.tex <==

\section{Introduction}

%% P1: Background
% 1. Definition of LLM, its characterisitics, its examples.
% 2. LLM capabilities and applications.
%%
Large Language Models (LLMs) are a type of advanced AI models designed to understand and generate human languages. LLMs are characterized by their massive scale, as they contain billions or even trillions of parameters and are trained on gigantic amount of data containing texts from a diverse range of sources. Some of the latest LLMs include GPT-series (e.g., GPT-3~\cite{Brown2020LanguageMA} and GPT-4~\cite{OpenAI2023GPT4TR}), Google-series (e.g., GLaM~\cite{Du2021GLaMES}, PaLM~\cite{Chowdhery2022PaLMSL}, and  PaLM-2~\cite{anil2023palm}), BLOOM~\cite{Scao2022BLOOMA1}, Meta-series (e.g., LLaMA 1$\&$2~\cite{Touvron2023LLaMAOA, Touvron2023Llama2O}), PanGu-$\sum$~\cite{Ren2023PanGuTT} and GLM~\cite{Zeng2022GLM130BAO}. \mz{Add Claude and Falcon}
%


Recently, we have witnessed significant advancement in Generative Artificial intelligence (AI). One of the major progress has been achieved in the realm of Large Language Models (LLMs)~\cite{OpenAI2023GPT4TR, Kaddour2023ChallengesAA, Zhao2023ASO, Yin2023ASO}, with ChatGPT attracted a substantial amount of attention across a variety of downstream applications such as natural language understanding (NLU), generation and complex reasoning~\cite{Yang2023HarnessingTP}, as well as domain-specific~\cite{wan2022g} tasks related to biomedical~\cite{Wang2021PretrainedLM, wan2023med}, law~\cite{Eliot2021GenerativePT} and code generation~\cite{Wei2022ChainOT, Chen2021EvaluatingLL}. The powerful knowledge storage and reasoning capabilities of LLMs benefit from their extremely large parameter and data scales~\cite{Kaplan2020ScalingLF, Hoffmann2022TrainingCL}. More specifically, model and data scaling not only achieves a significant capability improvement for pre-trained language models, but also exhibits emergent abilities~\cite{Wei2022EmergentAO} that are not observed in small-size language models (e.g., encoder-only BERT~\cite{Devlin2019BERTPO}, decoder-only GPT-1~\cite{Radford2018ImprovingLU}, encoder-decoder based BART~\cite{Lewis2019BARTDS}). 



%% P2: Motivation
% 1. Numbers related to efficiency.
%%the widespread adoption of these models has been hindered by . 
While LLMs are leading the next wave of AI revolution, the remarkable capabilities of LLMs come at the cost of their substantial resource demands~\cite{OpenAI2023GPT4TR, Du2021GLaMES, Chowdhery2022PaLMSL, Ren2023PanGuTT}. 
%
Figure~\ref{fig:carbon-performance} illustrates the relationship between model performance and the carbon emissions during training for LLaMA series LLMs. As shown, the amount of carbon emitted grows exponentially as the number of model parameter scales up.
%, . s disproportionately in relation to the performance of LLMs. 
%The high expense associated with training LLMs leads to a concentration of the development of powerful LLMs within major tech giants such as Google, OpenAI, and Meta. 
%
In additional to training, the inference demand significantly contributes to the operational cost of LLMs. With the rapid expension of applications and user base for LLMs, the energy and memory cost could exceed the training cost and become dominant factors for the overall environmental impact. As depicted in Figure~\ref{fig:speed-energy-memory}, more advanced LLMs exhibit higher memory and energy consumptions during inference. The persuit of better model also leads to the slowing down of genration, which needs to be addressed in the future.
% at inference time, running LLMs also consumes a lot of memory and energy, as depicted in Figure~\ref{fig:speed-energy-memory}. 
%
%Consequently, the deployment of LLMs typically requires powerful computational hardware and robust energy supply. This poses challenges for practical implementation of LLMs in edge or personalized devices. 

%%
Encouragingly, the considerable advancements in efficient LLMs have paved the way for a more inclusive deployment of these models. This progress facilitates the democratization of LLMs, expanding their utility to encompass training and inference in resource-constrained scenarios such as mobile devices and embedded systems.
%
These efforts not only make LLMs more accessible but also address environmental concerns related to energy use, which are crucial in an era of growing environmental concerns related to energy consumption \cite{chen2023maybe,schopf2023efficient,fisch2023towards}. 
%
Therefore, this paper predominantly centers on investigating techniques that enhance the efficiency of LLMs. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/LLMs_carbon-performance_cropped.pdf}
        % \vspace{-5mm}
	\caption{Illustrations of the peformance and carbon emissions for training LLMs of different scales. The reported performance is the average score of several commonsense reasoning benchmarks. The carbon emissions is estimated based on the GPU and time used for training the model. The size of each bubble corresponds to the number of model parameters. The original data can be found in~\cite{Touvron2023LLaMAOA, Touvron2023Llama2O}.}
	\label{fig:carbon-performance}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.75\textwidth]{Figures/LLMs_speed-energy-memory_cropped.pdf}
        % \vspace{-5mm}
	\caption{Energy consumption \textit{vs.} inference speed for various LLMs. The energy consumption and inference speed are measured on Nvidia A100-80GB GPUs with 16-bit floating point quantization. The size of each bubble corresponds to the memory (in Gigabytes) of each model. The original data can be found in~\cite{llm-perf-leaderboard}.}
	\label{fig:speed-energy-memory}
\end{figure}

\input{Section/framework}

The ambitious goal of democratizing Large Language Models (LLMs) cannot be realized without making substantial progress in concrete and specific methods for achieving efficiency. Unfortunately, a significant portion of the existing literature primarily focuses on discussions related to foundational models, specific tasks, evaluation benchmarks, practical applications, and alignment techniques for LLMs, as evidenced by the works~\cite{Zhao2023ASO, zha2023data, chang2023survey, wang2023aligning, kaddour2023challenges}. Alternatively, some literature only delves into particular aspects of efficiency, such as LLMs compression~\cite{zhu2023survey}, while others~\cite{zhuang2023survey, Tay2020EfficientTA} do not explicitly specify efficient approaches for LLMs, especially in cases where the model size exceeds 10 billion parameters. To foster a more comprehensive understanding of efficiency in LLMs, we systematically outline the current landscape of methodologies geared toward enhancing LLM efficiency. Additionally, we introduce an efficiency-driven taxonomy to categorize and organize the existing literature, as illustrated in Figure~\ref{fig:efficient LLMs structure}. Specifically, the strategies for achieving efficiency, stemming from the Model-Centric, Data-Centric, and Framework-Centric paradigms, play a pivotal role in the realm of efficient LLMs. Each of these approaches addresses distinct yet interconnected aspects, collectively contributing to the holistic development and utilization of efficient LLMs. We provide a high-level overview of these efficient methods below.


\begin{itemize}
    \item \textbf{Model-Centric Methods:} The Model-Centric perspective of efficient LLMs revolves around the central role of the LLM itself. It emphasizes model compression, efficient pre-training, efficient fine-tuning, efficient architecture design. In these approaches, the model is the focal point, and efforts are directed toward enhancing its capacity, adaptability, and performance. lightweight technologies, fine-tuning, and novel architectures fall within the purview of the Model-Centric paradigm.

    \item \textbf{Data-Centric Methods:} Orthogonally, the Data-Centric paradigm underscores the primacy of high-quality training and fine-tuning data. Here, the emphasis is on efficient data collection, curation, augmentation, and compression. A robust Data-Centric approach recognizes that the efficacy of LLMs largely hinges on the quality and quantity of the data they are trained on. Data selection, few-shot prompt, prompt compression and generation are fundamental components of this paradigm.

    \item \textbf{LLM Frameworks}: Notably, framework-Centric thinking broadens the perspective to encompass the overarching frameworks, libraries, and toolsets that facilitate the development and deployment of LLMs. It acknowledges the importance of the ecosystem in which LLMs operate, encompassing elements such as software infrastructure, libraries for model management, and deployment pipelines for efficient training or inference.

\end{itemize}

In sum, the necessity of Model-Centric, Data-Centric, and Framework-Centric aspects for LLMs lies in their complementary roles. The Model-Centric perspective enhances the model's intrinsic capabilities, the Data-Centric approach ensures the availability of high-quality training data, and the Framework-Centric paradigm provides the infrastructure for efficient model development and deployment. These facets collectively contribute to the holistic advancement of LLMs, allowing them to reach their full potential in various applications, from natural language understanding to creative text generation.








% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1\linewidth]{tree.pdf}
%   \vspace{-0.2in}
%   \caption {Overview of the efficient training of Large Language Models (LLMs), including computation efficiency, memory efficiency and hardware/algorithm co-design perspectives, efficient data-centric strategies so on. }
%   \vspace{-0.2in}
%   \label{fig:sample real data}
% \end{figure*}
% \vspace{-0.3mm}

%% P2: outline
% Need for efficient LLM
Despite the great success achieved through rapid development and numerous applications of LLMs, they still come with critical challenges stemming from the need of massive computation and memory resources for \textbf{pre-training} and \textbf{fine-tuning}, the high-latency for \textbf{inference}, and so forth. For example, the foundation model GPT-3~\cite{Brown2020LanguageMA}, equipped with $175$ billion parameters, was pre-trained on half a trillion tokens, which cost $335$ GPU-years or $28$ TFLOPS for V100 GPUs to train, and also require at least five $80$G A100 GPUs to deploy\zq{Reference?} \yuzheng{[How are they calculated? The original paper says "several thousand petaflop/s-days"]}. Beyond that, a more enormous language model PaLM $540$B~\cite{Chowdhery2022PaLMSL} consumed $6144$ TPU v4 chips and was pre-trained using nearly $780$ million natural language tokens. Apart from high pre-training cost, fine-tuning the entire LLMs for downstream tasks can be challenging and inefficient~\cite{Hu2023LLMAdaptersAA}, since it requires large memory to store billions of model parameters, activations, gradients, momentums, and so on. As a consequence, due to limited availability of GPU or TPU devices, it is infeasible for many practitioners to individually load and fine-tune LLMs on a specific downstream task.
Meanwhile, it is also worth noting that LLMs exhibit a high inference latency~\cite{Pope2022EfficientlyST}. \zq{This is due to the fact that (i) LLM's inference often generates one token at a step that results in low parallelism; (ii) the transient states during decoding lead to high memory occupation} (e.g., low parallelizability and large memory footprints), since the LLM's inference generates one token at a step and the transient states during decoding lead to high memory occupation \quanlu{Inference is bounded by memory bandwidth leading, which wastes the high parallelization of accelerators}. Furthermore, the considerable energy consumption of LLMs during training and inference contributes to a massive carbon footprint. Addressing this issue has become of paramount importance, focusing on rendering LLMs trainable with enhanced computational and energy efficiency as part of the Green AI~\cite{Georgiou2022GreenAD} initiative, while also democratizing access to these models within resource constraints. \yuzheng{[This paragraph is too long. It was written in the order of training, fine-tuning and inference. However the real challenges of LLMs (such as carbon emission and memory consumption) exists in in all 3 stages). I suggest to write his paragraph in the order of different challenges.]}

%% P3: Overview of the survey at a high level.
% 3 Tasks.
In order to address the above-mentioned challenges, researchers have proposed multiple efficient methods for training, fine-tuning, and inference for LLMs. These are part of the collaborate efforts to democratize LLMs and facilitate the widespread adoption of LLMs in real-world applications. 
\zq{Make sure this high-level summary concludes the discussed methods in a relatively comprehensive manner. Maybe discuss these methods in three aspects individually
These methods mainly include (i) \textit{Efficient training}, ; (ii)\textit{Efficient fine-tuning}, ; \textit{Efficient inference}}
They mainly involve reducing parameters size for inference (e.g., pruning~\cite{Frantar2023SparseGPTML, Sun2023ASA}, distillation~\cite{Gu2023KnowledgeDO, Huang2022IncontextLD} and MoE~\cite{Fedus2021SwitchTS, Shen2023MixtureofExpertsMI} \quanlu{seems MoE increases parameter size a lot}), reducing actual computation for training (e.g., quantization~\cite{Dettmers2023QLoRAEF, Dettmers2023QLoRAEF}), designing techniques to reduce memory~\cite{Dao2022FlashAttentionFA, Pagliardini2023FasterCA} \quanlu{quantization is also an effective way to reduce memory. A popular inference optimization for LLM is storing weights in 8 or 4 bits while computing with fp16, this is because LLM inference is memory bandwidth bound}, creating techniques for efficiently decoding-based inference~\cite{Liu2023DejaVC, Sheng2023HighthroughputGI}, and efficiently data-centric selection~\cite{Meng2022TuningLM, Zhou2023LIMALI} etc. The existing literature~\cite{Han2021PreTrainedMP, Zhou2023ACS, Qiu2020PretrainedMF, Wu2023ASO} has extensively explored the implementations and applications of pre-trained LLMs. In complement to these efforts, we contribute by systematically conducting a survey that examines these strategies from efficiency perspective. 

\zq{Do we include some accepted papers of NIPS2023?}

%%
\vspace{2mm}
\fakeparagraph{Major Contributions.}
%\subsection{Major Contributions}
Motivated by the need for efficient LLMs and the numerous attempts in previous researches, our primary aim is to thoroughly illuminate the accomplishments obtained in the domain of efficient techniques for LLMs. As shown in \figref{fig:sample real data} our survey provides a summary of these multi-aspect approaches. \zq{Maybe emphasize the advantages of our new category in comparison to the above naive category} We mainly categorize efficient LLMs techniques into two main categories, they are software designs encompassing efficient model-centric and data-centric methods, and software $\&$ hardware co-design including parallel training frameworks and hardware optimization strategies, respectively. Specifically, among these methods, (a) the \textbf{model-centric} perspectives include but not limited to memory-efficient model compression, efficient training, fine-tuning, inference, and efficient-attention backbones. (b) The \textbf{data-centric} views mainly focus on data selection, data compression, prompt engineering, data pre-processing, data augmentation, etc. Besides, (c) for \textbf{parallel training frameworks}, the solution involves data parallelism, tensor parallelism, and pipeline parallelism. (d) Regarding \textbf{hardware optimization strategies}, our survey will contain sparse matrix multiplication, mixed precision training, and hardware-aware efficient attention. \quanlu{What is the guideline for this classification? Seems model-centric and data-centric belong to the algorithm part? Parallel training framework and hardware optimization strategies are system part? They both contribute to efficient LLM.} Through this endeavor, our objective is to furnish a comprehensive snapshot of the current landscape of efficient LLMs, thereby empowering researchers and practitioners to navigate and facilitate the widespread adoption of LLMs.
\yuzheng{[I think this paragraph should be written based on Figure~\ref{fig:efficient LLMs structure}]}


The advent of LLMs has necessitated the development of specialized frameworks to efficiently handle their training, inference, and deployment. While mainstream libraries like TensorFlow, PyTorch, and JAX provide the foundations, they lack built-in support for specific optimizations and features crucial for LLMs. In Section 4, we describe existing frameworks tailored for LLMs, addressing their unique features, underlying libraries, and specializations.


%% P4: organization.
\vspace{2mm}
\fakeparagraph{Organization.}
%\subsection{Organization}
The rest of the survey is organized as follows.
\vspace{-0mm}
%\noindent \textbf{This survey is organized as follows:}
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{1.0pt}
   \setlength{\parsep}{1.0pt}
   \setlength{\parskip}{1.0pt}
    \item Section 2 discusses XXX provides a concise overview of recent background knowledge related to LLMs, encompassing their evolution, architecture, and specific capabilities. 
    
    \item Section 3 introduces XXX delve into the requisites, advanced methodologies, and challenges pertaining to the efficiency of LLMs, considering both software designs and soft-hardware co-designs.
    
     \item  Section 4 describes XXX 
     %an in-depth summary of evaluation metrics, benchmarks, and downstream applications for efficient LLMs will be presented.
    
    \item Section 5 XXX provide a comprehensive global perspective on efficient LLMs while accentuating potential future directions.
\end{itemize}




==> Section/2_Background.tex <==

\section{Background and Need for Efficient  Large Language Models}
\label{sec:LLM background}

%% Overview
In this section, we present an overview of cutting-edge Large Language Models (LLMs), all of which are based on the widely recognized Transformer architecture~\cite{Vaswani2017AttentionIA}. We first outline the foundational definition and developmental trajectory of LLMs. We then delve into the prevalent architectural variations and pre-training objectives that characterize LLMs. We also provide a succinct introduction to select capabilities and applications demonstrated by LLMs. Lastly, we explore the imperative role of resource-efficient LLMs in addressing societal needs.

\subsection{Background of Large Language Models}
Large Language Models (LLMs) are a type of advanced AI model designed to understand and generate human languages. They are characterized by their massive scale, as they contain more than billions of parameters and are trained on extensive data containing texts from a diverse range of sources. Some of the latest LLMs include GPT-series (e.g., GPT-3~\cite{Brown2020LanguageMA} and GPT-4~\cite{OpenAI2023GPT4TR}), Google-series (e.g., GLaM~\cite{Du2021GLaMES}, PaLM~\cite{Chowdhery2022PaLMSL}, and  PaLM-2~\cite{anil2023palm}), BLOOM~\cite{Scao2022BLOOMA1}, Meta-series (e.g., LLaMA~\cite{Touvron2023LLaMAOA} and LLaMA-2~\cite{Touvron2023Llama2O}), PanGu-$\sum$~\cite{Ren2023PanGuTT} and GLM~\cite{Zeng2022GLM130BAO}. \zq{Maybe add Claude and Falcon} Compared to small-scale language models~\cite{Devlin2019BERTPO, Radford2018ImprovingLU, Lewis2019BARTDS, Raffel2019ExploringTL}, recent studies on the \textbf{scaling laws} by \citet{Kaplan2020ScalingLF, Hoffmann2022TrainingCL, Clark2022UnifiedSL} demonstrate that pre-training LLMs with sufficient training data and extending the model size can largely enhance the performance of LLMs. Specifically, researchers from OpenAI~\cite{Kaplan2020ScalingLF} first investigated the power-law of cross-entropy loss with model size, dataset size, and the amount of computation resource. Their findings showed that larger models continually perform better and large model sizes may be more effective than big data, indicating that model parallelism is warranted.  Alternatively, DeepMind~\cite{Hoffmann2022TrainingCL} finds that current LLMs are significantly under-pre-trained and further proposes that the model size and the number of training tokens should be also scaled equally for compute-optimal training. Furthermore, \citet{Clark2022UnifiedSL} explore the scaling law on training routing networks for a mixture of experts (MoE) LLMs and found that the performance of all routing networks also follows the scaling law in the number of experts and in the underlying dense model size same as ~\cite{Kaplan2020ScalingLF}. \quanlu{SCALING LAWS FOR SPARSELY-CONNECTED FOUNDATION MODELS is another related work of scaling law} Apart from \textbf{model scaling}, ~\citet{Ren2023PanGuTT} clarify that \textbf{system scaling} is also crucial for LLMs, demonstrating that efficiently increasing the bandwidth between GPUs nodes and upgrading the computational ability of CPUs in the case of tensor~\cite{Shoeybi2019MegatronLMTM}  or pipeline parallelism~\cite{Huang2018GPipeET} is critical to the performance of LLMs. 
Consequently, the discovery of scaling law has played an important role in the fast advancement of LLMs, whose large capacity further underpins their capability to tackle intricate downstream tasks.

\samiul{I think we should consider that readers may not know much about LLMs and we need to make them familiar with LLMs and show how to distinguish LLMs from regular Transformer models. We should add a section here detailing the different mechanisms involved in LLM and why they are different from regular Transformer models. I suggest introducing some arenas where additional optimizations are required compared to regular transformers while outlining the standard training and inference process for LLMs}


\begin{table}[tp]
\centering
\caption{Summary of architectures, pre-training strategies, and representative models of LLMs.}
\vspace{-2mm}
\label{tab:llms}
\resizebox{1\textwidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
    \multicolumn{1}{c|}{\textbf{Architectures}} &\multicolumn{1}{c|}{\textbf{Pre-training Strategies}} & \multicolumn{1}{c}{\textbf{Models}}     \\ 
    \midrule
    \multirow{4}{*}{Decoder-only}  &     & \multirow{4}{6cm}{GPT-3, OPT, PaLM, BLOOM, MT-NLG,  GLaM,Gopher, chinchilla, LaMDA, GPT-J, LLaMA,  GPT-4, BloombergGPT} \\
                                                    
                                                         &  $-\sum_{i=1}^T log p(x_i|\{x_1, ..., x_{i-1}\})$,    \\
                                                        &   $\{x_1, ..., x_{T}\}$ is the input tokens               \\
                                                  &                                       \\
                                                  
    \midrule
    \multirow{2}{*}{Encoder-only}    &   $-\sum_{x \in mask(x)} log p(x|\hat{X})$,    & \multirow{2}{6cm}{BERT, RoBERTa, DistilBERT} \\ 
                                     & $\hat{X}$ is the sentence with masks,      & \\
    \midrule

    \multirow{2}{*}{prefix-decoder}    &    $-\sum_{i=1}^T log p(x_i|{P}, x_0, \cdots, x_{i-1})$, ${P}$ and   & \multirow{2}{6cm}{BERT, RoBERTa, DistilBERT} \\ 
                                     &$x=\{x_1,\cdots,x_T\}$ are the prefix tokens/predicted tokens      & \\
    \midrule

    \multirow{2}{*}{Encoder-decoder}    &    $-\sum_{i=1}^T log p(x_i|{X}, y_0, \cdots, y_{i-1})$,   & \multirow{2}{6cm}{BERT, RoBERTa, DistilBERT} \\ 
                                     &${X}$ and $Y=\{y_1,\cdots,y_T\}$ are the  input/predicted tokens      & \\
                    
    \bottomrule
    \end{tabular}
}
\end{table}

\begin{comment}
\subsection{Architectures and Pre-Training Strategies}

Pre-trained language models (PLMs) based on Transformer architectures are primarily classified into four categories: decoder-only, prefix-decoder, encoder-decoder, and encoder-only. These distinct architectures vary in their specific training strategies. In the following, we will elaborate on each of these four PLM architectures. The evolution of PLMs in various architectures are \red{shown in Fig. 2.}

\fakeparagraph{Decoder-Only Architecture.} Decoder-only architecture is currently the most dominant architecture for LLMs. This decoder architecture~\cite{Brown2020LanguageMA}, also known as auto-regressive language models, incorporates unidirectional casual mask attention strategy~\cite{Radford2018ImprovingLU}, i.e., the generated new token can only attend to previous tokens during pre-training in which the likelihood of the predicted token given the previous tokens is maximized. Examples of decoder-only LLMs includes GPT-3~\cite{Brown2020LanguageMA}, GPT-4~\cite{OpenAI2023GPT4TR}, LLaMA~\cite{Touvron2023LLaMAOA, Touvron2023Llama2O}, OPT~\cite{Zhang2022OPTOP}, GLaM~\cite{Du2021GLaMES}, PaLM~\cite{Chowdhery2022PaLMSL}, Gopher~\cite{Rae2021ScalingLM}, PanGu-$\sum$~\cite{Ren2023PanGuTT}, and GLM~\cite{Zeng2022GLM130BAO}. In contrast to encoder-only and encoder-decoder architectures, recently \citet{Wang2022WhatLM, Brown2020LanguageMA} suggest that the decoder-only architecture offers distinct advantages for LLMs. Specifically, decoder-only LLMs exhibit enhanced zero-shot generalization capabilities without requiring fine-tuning in downstream tasks. Moreover, the computational overhead associated with transfer learning using the decoder-only architecture is notably smaller compared to the encoder-decoder architecture. Additionally, the scaling laws~\cite{Kaplan2020ScalingLF, Hoffmann2022TrainingCL, Clark2022UnifiedSL} have predominantly been applied to decoder-only architectures, and empirical findings have shown that increasing the size of these architectures substantially enhances the reasoning capability of LLMs.

\fakeparagraph{Encoder-Only Architecture.} Encoder-only PLMs adopt Masked Language Modeling (MLM) to replace some ratio of tokens in the sequence with a special \texttt{[MASK]} token and pre-train a model to predict masked tokens in the sentence given the surrounding context to learn the semantic information via bi-directional attention. Notable examples of encoder-only PLMs include BERT~\cite{Devlin2019BERTPO}, RoBERTa~\cite{Liu2019RoBERTaAR}, ALBERT~\cite{Lan2019ALBERTAL}, ELECTRA~\cite{DBLP:conf/iclr/ClarkLLM20} and DeBERTa~\cite{He2020DeBERTaDB}. Although encoder-only architectures have achieved excellent results on natural language understanding (NLU) tasks, these architectures do not exhibit robust generalization capabilities comparable to the current prevailing decoder-only LLMs in zero-shot scenarios~\cite{Scao2022BLOOMA1}.

\fakeparagraph{Prefix-Decoder Architecture.} Prefix-decoder ~\cite{Raffel2019ExploringTL} represents a distinct variant of the decoder-only architecture. This specialized form extends decoder-only models by performing bidirectional attention over the prefix tokens and unidirectional attention on the predicted tokens. Without the prefix tokens, the architecture is equivalent to the standard 
auto-regressive language model. Through this way, prefix-decoder can both encode the prefix tokens and generate the new tokens one by one, sharing the same parameter. Typical prefix-decoder-based LLMs include CLM-130B~\cite{Zeng2022GLM130BAO} and U-PaLM~\cite{Tay2022TranscendingSL}.

\fakeparagraph{Encoder-Decoder Architecture.} 
In the encoder-decoder architecture, the encoder performs bi-directional attention computation on the input tokens. Then each layer of the decoder separately performs cross-attention computation on the latent embeddings from the encoder and autoregressively generates new tokens. Some PLMs are built based on the encoder-decoder architecture including BART~\cite{Lewis2019BARTDS}, T-5~\cite{Raffel2019ExploringTL} and Flan-T5~\cite{Chung2022ScalingIL}, etc. Compared to the decoder-only architecture, although pre-trained Language Models (PLMs) built on the encoder-decoder architecture have demonstrated more significant advancements in machine translation~\cite{Zhang2022ExaminingSA}, there are still few LLMs that are constructed based on the encoder-decoder architecture.
\end{comment}

\subsection{Capability of LLMs}
Scaling up LLMs can greatly improve performance and sample efficiency on a wide range of general downstream tasks, involving traditional NLU tasks (e.g., text classification, named entity recognition (NER), question answering, and entailment prediction)~\cite{Wang2018GLUEAM, Wang2019SuperGLUEAS, Rajpurkar2018KnowWY}, generation tasks (e.g., summarization, machine translation, and text or code generation)~\cite{Austin2021ProgramSW, Bojar2016FindingsOT, Chen2021EvaluatingLL}, knowledge-intensive tasks (e.g., open-domain question answering and massive multitask language understanding i.e., MMLU)~\cite{Kwiatkowski2019NaturalQA, Joshi2017TriviaQAAL, Hendrycks2020MeasuringMM}. However, when the language models are extended to a certain scale, specific \textit{emergent ability}~\cite{Wei2022EmergentAO} will surprisingly arise, which are not present in small models. In particular, the emergent ability for few-shot prompt-based task execution emerges when a model exhibits random performance up to a certain scale, beyond which its performance substantially surpasses random levels. The phenomenon is manifested in the following ways: (1) \textbf{Complex reasoning}. LLMs demonstrate state-of-the-art abilities in mathematical reasoning and common sense reasoning. The critical challenges of mathematical reasoning are the understanding of symbolic logic and multi-step reasoning. For instance, GPT-4~\cite{OpenAI2023GPT4TR} has outperformed task-specific methods on math benchmarks including GSM8k~\cite{Cobbe2021TrainingVT}, SVAMP~\cite{Patel2021AreNM} and AQuA~\cite{Ling2017ProgramIB}. Furthermore, the substantial knowledge capacity empowers LLMs to retain factual information and execute multiple inference steps concerning these facts. GPT-4 has also achieved remarkable results close to $100\%$ on StrategyQA~\cite{Geva2021DidAU} and ARC-C~\cite{Clark2018ThinkYH}. (2) \textbf{In-context learning (ICL)}. A very typical representation of emergent capabilities is the ability of in-context learning~\cite{Brown2020LanguageMA} discovered by GPT-3, different from supervised learning that needs to update model parameters, where LLMs make predictions only based on contexts augmented with a few examples using specific prompting template~\cite{Zhao2021CalibrateBU}. By adopting chain-of-thought (CoT)~\cite{Wei2022ChainOT, Zhang2022AutomaticCO} or tree-of-thought (ToT)~\cite{Yao2023TreeOT} prompting mechanism, the ICL ability can greatly assist LLMs in solving complex arithmetic reasoning via deriving intermediate reasoning for the final result. \citet{Wei2022ChainOT} hypothesize that the ICL ability stems from pre-training LLMs on the source code. (3) \textbf{Instruction-tuning}. Instruction-tuning aims to enhance the ICL ability of LLMs via training on human-level or task-specific instructions~\cite{Ouyang2022TrainingLM}. The technique can enable LLMs to follow the human instructions for new tasks without using explicit instances thus improve generalization ability of LLMs. Instruct-tuning researches contain InstructGPT~\cite{Ouyang2022TrainingLM}, APE~\cite{Zhou2022LargeLM} and Self-Instruct~\cite{Wang2022SelfInstructAL} etc. \red{Something about RLHF.}


\subsection{Need for Efficient LLMs}

While LLMs have indeed revolutionized the generative AI landscape, the widespread adoption of these models has been hindered by their substantial computational demands and extensive model parameters~\cite{OpenAI2023GPT4TR, Du2021GLaMES, Chowdhery2022PaLMSL, Ren2023PanGuTT}. \yuzheng{The remarkable capabilities of LLMs often comes at the expense of increased computational resources. Figure~\ref{fig:carbon-performance} indicates that the computational cost, as measured by the carbon emissions during training, grows disproportionately in relation to the performance of LLMs. The high expense associated with training LLMs leads to a concentration of the development of powerful LLMs within major tech giants such as Google, OpenAI, and Meta. At inference time, running LLMs also consumes a lot of memory and energy, as depicted in Figure~\ref{fig:speed-energy-memory}. Consequently, the deployment LLMs typically requires powerful computational hardware and robust energy supply. This poses challenges for practical implementation of LLMs in edge or personalized devices.} Encouragingly, the considerable advancements in efficient LLMs have paved the way for a more inclusive deployment of these models. This progress facilitates the democratization of LLMs, expanding their utility to encompass training and inference in resource-constrained scenarios such as mobile devices and embedded systems.
%
Therefore, this paper predominantly centers on investigating techniques that enhance the efficiency of LLMs. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.75\textwidth]{Figures/LLMs_carbon-performance_cropped.pdf}
        % \vspace{-5mm}
	\caption{Illustrations of the peformance and carbon emissions for training LLMs of different scales. The reported performance is the average score of several commonsense reasoning benchmarks. The carbon emissions is estimated based on the GPU and time used for training the model. The size of each bubble corresponds to the number of model parameters. The original data can be found in~\cite{Touvron2023LLaMAOA, Touvron2023Llama2O}.}
	\label{fig:carbon-performance}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.9\textwidth]{Figures/LLMs_speed-energy-memory_cropped.pdf}
        % \vspace{-5mm}
	\caption{Energy consumption \textit{vs.} inference speed for various LLMs. The energy consumption and inference speed are measured on Nvidia A100-80GB GPUs with 16-bit floating point quantization. The size of each bubble corresponds to the memory (in Gigabytes) of each model. The original data can be found in~\cite{llm-perf-leaderboard}.}
	\label{fig:speed-energy-memory}
\end{figure}

\input{Section/framework}

\subsection{Tasks in Efficient LLMs}

% \mz{
% Here we provide an overview of all the 3 major tasks: data-centric, model-centric, and frameworks. Within each task, we list all the subtasks. Pls refer to section 2.3 of https://arxiv.org/abs/2303.10158. Here we refer to Figure 1.
% } 

The ambitious goal of democratizing Large Language Models (LLMs) cannot be realized without making substantial progress in concrete and specific methods for achieving efficiency. Unfortunately, a significant portion of the existing literature primarily focuses on discussions related to foundational models, specific tasks, evaluation benchmarks, practical applications, and alignment techniques for LLMs, as evidenced by the works~\cite{Zhao2023ASO, zha2023data, chang2023survey, wang2023aligning, kaddour2023challenges}. Alternatively, some literature only delves into particular aspects of efficiency, such as LLMs compression~\cite{zhu2023survey}, while others~\cite{zhuang2023survey, Tay2020EfficientTA} do not explicitly specify efficient approaches for LLMs, especially in cases where the model size exceeds 10 billion parameters. To foster a more comprehensive understanding of efficiency in LLMs, we systematically outline the current landscape of methodologies geared toward enhancing LLM efficiency. Additionally, we introduce an efficiency-driven taxonomy to categorize and organize the existing literature, as illustrated in Figure~\ref{fig:efficient LLMs structure}. Specifically, the strategies for achieving efficiency, stemming from the Model-Centric, Data-Centric, and Framework-Centric paradigms, play a pivotal role in the realm of efficient LLMs. Each of these approaches addresses distinct yet interconnected aspects, collectively contributing to the holistic development and utilization of efficient LLMs. We provide a high-level overview of these efficient methods below.


\begin{itemize}
    \item \textbf{Model-Centric Methods:} The Model-Centric perspective of efficient LLMs revolves around the central role of the LLM itself. It emphasizes model compression, efficient pre-training, efficient fine-tuning, efficient architecture design. In these approaches, the model is the focal point, and efforts are directed toward enhancing its capacity, adaptability, and performance. Lightweight technologies, Fine-tuning, and novel architectures fall within the purview of the Model-Centric paradigm.

    \item \textbf{Data-Centric Methods:} Orthogonally, the Data-Centric paradigm underscores the primacy of high-quality training and fine-tuning data. Here, the emphasis is on efficient data collection, curation, augmentation, and compression. A robust Data-Centric approach recognizes that the efficacy of LLMs largely hinges on the quality and quantity of the data they are trained on. Data selection, few-shot prompt, prompt compression and generation are fundamental components of this paradigm.

    \item \textbf{LLM Frameworks}: Notably, framework-Centric thinking broadens the perspective to encompass the overarching frameworks, libraries, and toolsets that facilitate the development and deployment of LLMs. It acknowledges the importance of the ecosystem in which LLMs operate, encompassing elements such as software infrastructure, libraries for model management, and deployment pipelines for efficient training or inference.

\end{itemize}

In sum, the necessity of Model-Centric, Data-Centric, and Framework-Centric aspects for LLMs lies in their complementary roles. The Model-Centric perspective enhances the model's intrinsic capabilities, the Data-Centric approach ensures the availability of high-quality training data, and the Framework-Centric paradigm provides the infrastructure for efficient model development and deployment. These facets collectively contribute to the holistic advancement of LLMs, allowing them to reach their full potential in various applications, from natural language understanding to creative text generation.



==> Section/Benchmark.tex <==

\section{Benchmarks}

Benchmarks

==> Section/Discussion.tex <==

\section{Discussion and Future Directions}

The exploration into efficient techniques for LLMs is essential given the burgeoning size of these models and their computational demands. Some prospective research directions, including efficient multi-modal LLMs and benchmarks for evaluating efficient LLMs, are highlighted below:
%\begin{itemize}
    %\item 

\vspace{1mm} 
\noindent
\textbf{Standardized Benchmark for Efficient LLM Techniques. }As the field of efficient strategies for LLMs progresses, having robust and fair benchmarks and evaluation metrics is indispensable. These benchmarks can provide a standardized platform to assess the efficiency of LLMs comprehensively, covering aspects like computational cost, memory footprint, energy consumption, and performance across diverse tasks. This will enable a clearer understanding of the trade-offs involved and help guide the community towards more efficient and environmentally sustainable model designs.

\vspace{1mm}
\noindent
    %\item 
\textbf{Efficient Multi-modal LLMs. }Efficient techniques are not only crucial for monolithic LLMs but also for multi-modal LLMs~\cite{yin2023survey, wan2023med} that integrate information across text, image, and sometimes audio or video data. Efficient multi-modal LLMs have the potential to unlock new dimensions of understanding by leveraging complementary information from different modalities. Research towards optimizing the interaction between modalities and reducing the computational overhead of multi-modal fusion for low-resource machine is vital.

%\end{itemize}
